Self-supervised Speaker Recognition Training Using Human-Machine Dialogues

Speaker recognition, recognizing speaker identities based on voice alone, enables important downstream applications, such as personalization and authentication. Learning speaker representations, in the context of supervised learning, heavily depends on both clean and sufficient labeled data, which is always difficult to acquire. Noisy unlabeled data, on the other hand, also provides valuable information that can be exploited using self-supervised training methods. In this work, we investigate how to pretrain speaker recognition models by leveraging dialogues between customers and smart-speaker devices. However, the supervisory information in such dialogues is inherently noisy, as multiple speakers may speak to a device in the course of the same dialogue. To address this issue, we propose an effective rejection mechanism that selectively learns from dialogues based on their acoustic homogeneity. Both reconstruction-based and contrastive-learning-based self-supervised methods are compared. Experiments demonstrate that the proposed method provides significant performance improvements, superior to earlier work. Dialogue pretraining when combined with the rejection mechanism yields 27.10% equal error rate (EER) reduction in speaker recognition, compared to a model without self-supervised pretraining.

==> 99_rejection.tex <==
\section{Self-supervised Rejection}
\label{subsec:emb_fusion}

Our dialogue dataset also contains some utterances with multiple speakers and/or some strong background noise which may affect the quality of learning. In other words, since the model will try to distinguish all the given training data as good as possible, multi-speaker examples may push neural network to learn some non-robust and SID-unrelated features. In order to resolve the issue of noisy dialogues consisting of multiple speakers, we propose a self-supervised rejection mechanism such that the neural network decides how much weigh each dialogue's contribution to the final loss. Computation of the weights are simply using pair-wise similarity between the dialogue utterances, this way we compute a compactness metric for each dialogue constructing the batch. We scale each loss computed using dialogues with the compactness value computed. We propose two different rejection mechanism which we call hard rejection and soft rejection. Depending on the utterance embeddings we compute the pairwise cosine similarities and if the computed similarity is lower than predefined rejection threshold, we eliminate the dialogue. For instance, if we set the rejection threshold to 0.5 then it means we reject all the dialogues with lower compactness than 0.5. 

Let $\mathbf{u}$ be the batch of utterances where $u_{11}$ and $u_{12}$ are coming from first dialogue. Then we get our embeddings by passing the batch through our encoder.
\begin{equation}
\begin{aligned}
\mathbf{u} &= [u_{11} \; u_{12} \; u_{21} \; u_{22} \; ... \; u_{n2}]^{T} \\
 \mathbf{x} &= f(\mathbf{u}) = [x_{11} \; x_{12} \; x_{21} \; x_{22} \; ... \; x_{n2}]^{T}
 \end{aligned}
\end{equation}

We define the compactness of each dialogue as the pairwise-similarity between the utterances coming from the same dialogue what we also call positive pair compactness.
 \begin{equation}
\begin{aligned}
c_{i}&=s(x_{i1}, x_{i2}) = \frac{x_{i1}^Tx_{i2}}{||x_{i1}|| \cdot ||x_{i2}||} \\
\mathbf{c} &= [c_{1} \; c_{2} \; c_{3} \; ... \; c_{n}]^{T} 
\end{aligned}
\end{equation}

Then the individual loss corresponding for i'th dialogue can be computed using cross entropy as follow:
 \begin{equation}
l_i = -\log\frac{\exp(s(x_{i.}, x_{i.}))}{\sum_{j=1}^{n}\exp(s(x_{i.}, x_{j.}))} 
\end{equation}

On the other hand, if we incorporate the hard rejection mechanism along with loss computation we get rejection loss as follow:

 \begin{equation}
\begin{aligned}
l_i^r &= -\log\frac{\exp(s(x_{i.}, x_{i.}))}{\sum_{j=1,c_j>t}^{n}\exp(s(x_{i.}, x_{j.}))} \; \text{if} \; c_i>t \; \text{else} \; 0 \\
\mathbf{l} &= [l_{1} \; l_{2} \; ... \; l_{n}]^{T}  \\
\mathbf{l}^r &= [l_{1}^r \; l_{2}^r \; ... \; l_{n}^r]^{T} \\
\mathbf{L^*} &= \sum \mathbf{l}^r \\
\end{aligned}
\end{equation}
